D-branes and Non-Perturbative Quantum Field Theory: Stringy Instantons and Strongly Coupled Spintronics

The non-perturbative dynamics of quantum field theories is studied using theoretical tools inspired by string formalism. Two main lines are developed: the analysis of stringy instantons in a class of four-dimensional N=2 gauge theories and the holographic study of the minimal model for a strongly coupled unbalanced superconductor. The field theory instanton calculus admits a natural and efficient description in terms of D-brane models. In addition, the string viewpoint offers the possibility of generalizing the ordinary instanton configurations. Even though such generalized, or stringy, instantons would be absent in a purely field-theoretical, low-energy treatment, we demonstrate that they do alter the IR effective description of the brane dynamics by introducing contributions related to the string scale. In the first part of this thesis we compute explicitly the stringy instanton corrections to the effective prepotential in a class of quiver gauge theories. In the second part of the thesis, we present a detailed analysis of the minimal holographic setup yielding an effective description of a superconductor with two Abelian currents. The model contains a scalar field whose condensation produces a spontaneous symmetry breaking which describes the transition to a superfluid phase. This system has important applications in both QCD and condensed matter physics; moreover, it allows us to study mixed electric-spin transport properties (i.e. spintronics) at strong coupling.

==> QNM.tex <==
For an AdS black hole, i.e. a blak hole in an asymptotically AdS spacetime, the QNM are defined
as the solutions of the wave equation which satisfie the in-going boundary condition at the horizon
and a vanishing Dirichlet boundary condition at the conformal boundary.

==> dila.tex <==
The dilaton corresponds to the massless scalar mode in the closed-string spectrum.
Close strings propagate in the whole ambient spacetime, so we can consider the presence of a non-trivial expectation
value for the dilaton. In other term we can study string scattering in the presence of a background value of the dilaton, \cite{Becker:2007zj}.
This possibility is realized considering a new term in the worldsheet action, namely
\begin{equation}\label{ilatone}
 S_{\text{dil}} = \int_{\Sigma} d^2 \sigma \sqrt{h} \Phi(x) R(x) \ ,
\end{equation}
where $R$ is the Ricci scalar associated to the worldsheet metric $h$.
In the expression of the dilaton, let us separate the VEV $\phi$ and the fluctuations $\Delta(x)$ 
\begin{equation}
 \Phi(x) = \phi + \Delta(x)\ .
\end{equation}
Eq.\eqref{ilatone} becomes
\begin{equation}
 S_{\text{dil}} = \int_{\Sigma} d^2 \sigma \sqrt{h} \phi R(x) + \int d^2 \sigma \sqrt{h} \Delta(x) R(x)\ .
\end{equation}
The term depending on $\phi$ is topological and can be rewritten in terms of the Euler number $\chi$:
\begin{equation}
 S_{\text{dil}}\big|_{\phi} = \int_{\Sigma} d^2 \sigma \sqrt{h} \phi R(x) = \phi \ \chi(\Sigma) = \phi (2 - 2n_h).
\end{equation}
where $n_h$ is the number of handles (here we are considering just topologies without boundaries or crosscaps).
In the expansion of the string partition function according to the topologies of the worldsheet
\begin{equation}
 Z = \sum_{n_h = 0}^\infty Z_{n_h}
\end{equation}
we have that each term $Z_{n_h}$ contains
\begin{equation}
 (e^{-S_{\text{dil}}}) \propto e^{\phi(2n_h-2)}.
\end{equation}
It is then natural to relate the topology expansion to a perturbative expansion where $\phi$ is related to the coupling constant (according to which we expand perturbatively)
in the following way:
\begin{equation}
 g_s = e^{\phi}.
\end{equation}
Notice that the introduction of a handle contributes a factor $g_s^2$.
In the field theory limit the introduction of a handle corresponds to introducing a four fields interaction vertex.


==> inmath.tex <==
The gauge field is a connection over the base manifold representing spacetime.
In particular, the gauge instantons and anti-instantons considered in theoretical physics are self-dual and anti-self-dual 
connections on the $4$-dimensional Euclidean space.
The instanton moduli parameterizing the global characteristics of instantons
form a topological space possessing a rich structure.
It is from a deep study of the moduli space of instantons that some geometrical features of 4-manifolds
could be analyzed\footnote{A $4$-manifold is a $4$-dimensional differentiable manifold (WARNING).}.
More precisely, from considering the Yang-Mills instanton moduli space one can define geometrical invariant quantities
that depend on the differentiable structure of the base $4$-dimensional manifold.
The first works performed using such methods inspired by theoretical physics into the context of topological 
and geometrical features of $4$-manifolds
were proposed by Donaldson in the middle $80$'s.
One of his main results implies the existence of a kind of $4$-manifolds that can be showed to be topologically 
even though not differentiably equivalent to the $4$-dimensional Euclidean space $\mathbb{R}^4$.
Such spaces are usually referred to as ``exotic''\footnote{Note that they have nothing to do with the exotic
instantons of which we are going to speak abundantly in the following, \ref{mio1}.}. 
Their exotic character consists in the bizarre property that they possess compact subsets that cannot
be contained within any differentiably embedded $3$-sphere.
This opposes what instead happens for standard $\mathbb{R}^4$.
For a discursive account of this topic look at \cite{Atiyah:1986pr}.

==> math.tex <==



